Simultaneous Color Computer Generated Holography

Computer generated holography has long been touted as the future of augmented and virtual reality (AR/VR) displays, but has yet to be realized in practice. Previous high-quality, color holographic displays have made either a 3$\times$ sacrifice on frame rate by using a sequential color illumination scheme or used more than one spatial light modulator (SLM) and/or bulky, complex optical setups. The reduced frame rate of sequential color introduces distracting judder and color fringing in the presence of head motion while the form factor of current simultaneous color systems is incompatible with a head-mounted display. In this work, we propose a framework for simultaneous color holography that allows the use of the full SLM frame rate while maintaining a compact and simple optical setup. Simultaneous color holograms are optimized through the use of a perceptual loss function, a physics-based neural network wavefront propagator, and a camera-calibrated forward model. We measurably improve hologram quality compared to other simultaneous color methods and move one step closer to the realization of color holographic displays for AR/VR.

==> 08_cut_sections.tex <==
% I don't think we need the partial coherence in the lit review since it's not that important to the method and we site them later

\paragraph{Incoherent and Partially Coherent Holography}
\label{Coherence}
Traditional holography has been performed with strongly coherent light sources leading to distracting speckle in the holograms formed.
%
Additionally, these coherent light sources are typically lasers which pose danger to the eyes
%
Recent work has investigated the feasibility of using partially coherent and incoherent light sources such as SLEDs and LEDs \cite{Deng2017CoherenceDisplays}.
%
\fs{Can LED really be called incoherent? Dont they still have a big spatial coherence, just poor temporal coherence?}
%
\cite{Peng2021Speckle-freeCalibration} models the partially coherent light source simply as the summation of coherent light sources.
%
Using this model produces holograms with significantly reduced speckle leading to sharp, high contrast images.
%
Speckle reduction is of particular importance for color holography as the speckle from each color channel is not aligned. 
%
This leads to mismatching of color balancing and the production of sepia toned holograms.
%
\fs{It's not really clear why you mention partial coherent holography here. Can you maybe explain a bit what implications this might have for your algorithm/work?}

\subsection{Active Camera-in-the-Loop}

\todo{This section is on hold, pending if we use active CiTL in image capture tomorrow. Below is text already written about CiTL which needs to be condensed into a few sentences if we're using it.}

% \gk{ from related work:
% As previously mentioned, small model mismatch often leads to large artifacts in CGH\cite{Peng2020NeuralTraining}.
% %
% While including a neural network in the forward model makes dramatic improvement, it still leaves room for image quality improvement.
% %
% In order to further reduce this detrimental model mismatch, SLM patterns can be optimized with what is known as a camera in the loop strategy. 
% %
% This strategy consists of both computationally and physically propagating the modified wave front. 
% %
% By propagating the wavefront computationally, the computational graph is created allowing for backpropagation to be used for SLM pattern optimization later. 
% %
% The result of the computational propagation is replaced, however, with the captured physical propagation before backpropagation is performed.
% %
% While this does not change the underlying calculation for the gradients, it can change the scale and even the sign of the gradients \cite{Peng2020NeuralTraining, Peng2021Speckle-freeCalibration,Chakravarthula2020LearnedDisplays, Mosleh2020Hardware-in-the-LoopPipelines, Chen2022Off-axisGeneration} .
% %
% This gradient modification allows for the experimentally captured hologram to be iteratively improved upon achieving excellent image quality.}

% \gk{this section should be compressed}



